Transport coefficients associated to black holes on the brane: analysis of the shear viscosity-to-entropy density ratio

In this thesis, we apply the AdS/CFT correspondence to space-times associated with extensions of General Relativity. We are particularly interested in calculating the transport coefficient, the shear viscosity, associated with the effective field theory whose dual is a black hole space-time in bulk. The correspondence also allows us to compute thermodynamic quantities, in which the entropy, plays a prominent role when the ratio between the shear viscosity-to-entropy density is taken. This ratio is conjectured to have a minimum value of $1/4{\pi}$, in natural units. The main results presented in this thesis consist of calculating the ratio for two different cases, and then applying the KSS conjecture - which establishes the minimum value for the ratio -, to investigate properties associated with the deformed space-time metrics. A brief review of General Relativity and Black Holes is presented. The so-called Brane World formalism is introduced, obtaining the equivalent of Einstein's equations and Black Hole solutions on the brane, which can be seen as extensions of solutions known in General Relativity. We discuss the formulation of AdS/CFT correspondence, and how to apply it to compute transport coefficients. Then applying this knowledge to compute transport coefficients associated with the solutions constituting an extension of General Relativity. Naturally, throughout the process of developing this work other interesting questions arise, therefore we include two studies related to these developments. In one we investigate the computation of transport coefficients when we have a fermionic sector in the model. The second is a proposal on how to evaluate the consistency of AdS/CFT correspondence via the calculation of the Weyl anomaly.

==> chapters/GR.tex <==
\newpage
\chapter{General Relativity} \label{part:1}

%%%%% brief introduction
\par The General Theory of Relativity is currently the standard description of gravity. It was first presented to the community in 1915 by Albert Einstein \cite{Einstein:1915by} as a generalisation of his theory of Special Relativity. In fact, General Relativity (GR) is a theory about space-time rather than gravity itself, whereas gravity emerges as a feature of space-time, namely: curvature. There is a wide range of applications of this theory, from understanding the nature of space-time itself and the gravitational interaction at the classical level, celestial motion, astrophysics, evolution and stability of stars, galaxies, black holes and cosmology.

\par In the last 20 years or so, GR has also caught attention from a different public, the Condensed Matter community. The publication by Juan Maldacena in 1997 \cite{Maldacena:1997re} has conjectured the duality between Conformal Field Theories and a very specific kind of solution of GR, the so called Anti-de Sitter space-time. Through this duality it is possible to study, amongst other things, strongly coupled condensed mater systems, making it possible to unveil physics that cannot be described otherwise.

\par This chapter is an introduction to the basic features of GR, needed to explore the realm of AdS/CMT. It is not intended to be an introduction of GR \textit{per se}, instead, it is presented such that instrumental use of the theory can be made in a consistent manner in future chapters. For an introductory level there are two references which have shown to be very useful to the writer, these are books from Bernard Schutz \cite{Schutz:1985jx} and Sean Carroll \cite{Carroll:2004st}. Both books cover GR from scratch and require a minimum amount of knowledge to be understood, these are intended to the reader with no familiarity at all with GR. More advanced books in the subject are the ones from Wald \cite{Wald:1984rg}, MTW \cite{Misner:1974qy}, Weinberg \cite{Weinberg:1972kfs} and Hawking\&Ellis \cite{Hawking:1973uf}. These contain a formal approach to the subject, and explore deeply the features of the theory. It is also worth to mention a useful handbook of GR that is a manual of solutions, which is always useful.

%%%%section 1
\section{The Einstein-Hilbert action}
\par Usually there are two different ways of presenting GR, one consists of introducing a good amount of Differential Geometry and then argue why some choices are suitable for describing gravity. The other is a more direct approach and is the one we choose here, which is starting from a given action and deriving properties about it. 

\subsection{Mathematical preliminaries}

\par This is a very short summary of the mathematics of GR. It is by no means intended to be a formal introduction, but rather a short summary of the basic properties and expressions of tensors that will appear in the next sections. It is instructive to recall some notions of geometry before presenting the action and deriving the equations of motion.

\par Throughout this chapter only pseudo-Riemannian manifolds are considered, the pseudo indicates a minus sign in one component of the metric tensor, which we now proceed to describe. The metric tensor encodes all properties of the geometry, from the metric tensor quantities such as the connection and curvature can be calculated. Formally it is called the First Fundamental Form of the manifold, and characterises the inner product, i.e. defines angles and lengths. For instance, consider the inner product of Special Relativity between four-vectors $A^{\mu}$ and $B^{\mu}$
\begin{equation} \label{eq:1}
A_{\mu}B^{\mu}=-A_{0}B^{0}+A_{i}B^{i}\ .
\end{equation}
In Eq. \eqref{eq:1} the metric is given by $\eta_{\mu\nu}=\text{diag}\left(-1,+1,+1,+1\right)$, the well known Minkowski metric. GR generalizes this notion and allows the components of the metric to be functions of the coordinates as well as not necessarily diagonal. A generic space-time metric will have its components denoted by $g_{\mu\nu}\equiv g_{\mu\nu}\left(x^{\mu}\right)$ and the following properties hold
\begin{align}
\begin{aligned}
g_{\mu\nu}=g_{\nu\mu} \ , \ \ \ \
g_{\mu\lambda}g^{\lambda\nu}=\delta_{\nu}^{\mu}\ ,
\end{aligned}
\end{align}
i.e. it is symmetric and invertible.

\par Upon generalisation of the metric, one needs to introduce the covariant derivative, $\nabla_{\mu}$, as a replacement for the ordinary derivative $\partial_{\mu}$. It is necessary, in order to define parallelism and transport of vectors from one point to another in the manifold. From an intuitive point of view, one can think about the covariant derivative as an ordinary derivative plus a correction term that accounts for the change in the vector itself due to it being moved from one point to another in the manifold. Denoting a vector by $A^{\mu}$, its covariant derivative is defined by
\begin{equation} \label{eq:2}
	\nabla_{\nu}A^{\mu}=\partial_{\nu}A^{\mu}+\Gamma_{\nu\lambda}^{\mu}A^{\lambda} \ .
\end{equation}
Similarly, let $A_{\mu}$ be a covector and $A^{\mu}_{\nu}$ a mixed tensor, the covariant derivative acts like
\begin{align}
	\nabla_{\nu}A_{\mu}=\partial_{\nu}A_{\mu}-\Gamma_{\nu\mu}^{\rho}A_{\rho}	\label{eq:3}\ ,			\ \ \ \
	\nabla_{\lambda}A_{\text{ }\nu}^{\mu}=\partial_{\lambda}A_{\text{ }\nu}^{\mu}+\Gamma_{\lambda\rho}^{\mu}A_{\text{ }\nu}	^{\rho}-\Gamma_{\lambda\nu}^{\rho}A_{\text{ }\rho}^{\mu}  \ . %\label{eq:4}
\end{align} 
And so on for different combinations of indices in all sorts of tensors.

\par At this point it should be emphasised that $\Gamma_{\nu\lambda}^{\mu}$ is only a connection that accounts to transporting the vector. Let $a,b\in\mathbb{R}$, $\varphi\equiv\varphi(x^{\mu})$ a scalar field, and $A,B$ be vectors or tensors, so the covariant derivative satisfies the four properties:
\begin{itemize}
\item Linearity: $\nabla\left(aA+bB\right)=a\nabla A+b\nabla B$.
\item Acts as the regular derivative on scalar fields: $\nabla\varphi=\partial\varphi$.
\item Obeys Leibniz rule: $\nabla\left(AB\right)=\left(\nabla A\right)B+A\left(\nabla B\right)$.
\item Metric compatibility: $\nabla_{\lambda}g_{\mu\nu}$.
\end{itemize}

\par Consider the commutator of covariant derivatives, as given in Eq. \eqref{eq:2}, acting on a vector field $A^{\mu}$:
\begin{equation} \label{eq:5}
	\left[\nabla_{\mu},\nabla_{\nu}\right]A^{\lambda}=R_{\text{ }\mu\nu\rho}^{\lambda}A^{\rho}+T_{\text{ }\mu\nu}^{\rho}\nabla_{\rho}V^{\lambda}\ ,
\end{equation}
the first term is the Riemann tensors contracted with the vector, whereas the second one is the torsion tensor. This relation enables one to extract all the relevant geometric quantities from knowledge of the covariant derivative operator. Put in other words, given the connection $\Gamma$ all geometric properties of a manifold can be obtained.

\par There are several ways of deriving the GR connection, the so called Levi-Civita connection, or sometimes Christoffel connection. The argument given here is the simplest one for time sake, the interested reader is referred to one of the references in the beginning of this chapter for other, more physically intuitive, derivations.

\par There is a theorem \cite{RicciTheoremBook}  that establishes that torsion and curvature are uniquely defined by the connection, this fact enables a significant simplification. It is widely known in GR that torsion plays no role at all in the theory, and all the geometric effects are related to curvature. This is, of course, a choice - a wise one, but nonetheless a choice -, that simplifies a lot the expressions. From this theorem there is one, and only one, connection that accounts for zero torsion in Eq. \eqref{eq:5} and it is given by:
\begin{equation} \label{eq:6}
	\Gamma_{\mu\nu}^{\lambda}=\frac{1}{2}g^{\lambda\rho}\left(\partial_{\mu}g_{\rho\mu}+\partial_{\nu}g_{\nu\rho}-\partial_{\rho}g_{\mu\nu}\right) \ .
\end{equation}
As one can easily check, this connection is symmetric and thus, makes the second term in Eq. \eqref{eq:5} vanish. Eq. \eqref{eq:6} can be derived directly from the metric compatibility condition once it is assumed that $\Gamma_{\mu\nu}^{\lambda}=\Gamma_{\nu\mu}^{\lambda}$.

\par Using Eq. \eqref{eq:6} in Eq. \eqref{eq:5} one can derive the explicit expression for the Riemann tensor (recall that the torsion vanishes identically)
\begin{align*}
\begin{aligned}
	\left[\nabla_{\mu},\nabla_{\nu}\right]V^{\lambda}&=\nabla_{\mu}\left(\nabla_{\nu}V^{\lambda}\right)-\nabla_{\nu}\left(\nabla_{\mu}V^{\lambda}\right)\\
	&=\partial_{\mu}\nabla_{\nu}V^{\lambda}-\Gamma_{\mu\nu}^{\rho}\nabla_{\rho}V^{\lambda}+\Gamma_{\mu\rho}^{\lambda}\nabla_{\nu}V^{\rho}-\partial_{\nu}\nabla_{\mu}V^{\lambda}+\Gamma_{\mu\nu}^{\rho}\nabla_{\rho}V^{\lambda}-\Gamma_{\nu\rho}^{\lambda}\nabla_{\mu}V^{\rho}\\
	&=\partial_{\mu}\left(\partial_{\nu}V^{\lambda}+\Gamma_{\nu\theta}^{\lambda}V^{\theta}\right)-\Gamma_{\mu\nu}^{\rho}\left(\partial_{\rho}V^{\lambda}+\Gamma_{\rho\theta}^{\lambda}V^{\theta}\right)+\Gamma_{\mu\rho}^{\lambda}\left(\partial_{\nu}V^{\rho}+\Gamma_{\nu\theta}^{\rho}V^{\theta}\right)\\
	&-\partial_{\nu}\left(\partial_{\mu}V^{\lambda}+\Gamma_{\mu\theta}^{\lambda}V^{\theta}\right)+\Gamma_{\mu\nu}^{\rho}\left(\partial_{\rho}V^{\lambda}+\Gamma_{\rho\theta}^{\lambda}V^{\theta}\right)-\Gamma_{\nu\rho}^{\lambda}\left(\partial_{\mu}V^{\rho}+\Gamma_{\mu\theta}^{\rho}V^{\theta}\right)\\
	&=\partial_{\mu}\Gamma_{\nu\theta}^{\lambda}V^{\theta}-\partial_{\nu}\Gamma_{\mu\theta}^{\lambda}V^{\theta}+\Gamma_{\mu\rho}^{\lambda}\Gamma_{\nu\theta}^{\rho}V^{\theta}-\Gamma_{\nu\rho}^{\lambda}\Gamma_{\mu\theta}^{\rho}V^{\theta}\\
	&=\left(\partial_{\mu}\Gamma_{\nu\theta}^{\lambda}-\partial_{\nu}\Gamma_{\mu\theta}^{\lambda}+\Gamma_{\mu\rho}^{\lambda}\Gamma_{\nu\theta}^{\rho}-\Gamma_{\nu\rho}^{\lambda}\Gamma_{\mu\theta}^{\rho}\right)V^{\theta}\\
	&=R_{\text{ }\theta\mu\nu}^{\lambda}V^{\theta}
\end{aligned}
\end{align*}
i.e. 
\begin{equation} \label{eq:7}
R_{\text{ }\theta\mu\nu}^{\lambda}=\partial_{\mu}\Gamma_{\nu\theta}^{\lambda}-\partial_{\nu}\Gamma_{\mu\theta}^{\lambda}+\Gamma_{\mu\rho}^{\lambda}\Gamma_{\nu\theta}^{\rho}-\Gamma_{\nu\rho}^{\lambda}\Gamma_{\mu\theta}^{\rho}\ .
\end{equation}
The Ricci tensor is defined from the Riemann tensor by the contraction
\begin{equation} \label{eq:8}
	R_{\mu\nu}=R_{\text{ }\mu\lambda\nu}^{\lambda}\ .
\end{equation}
And taking the trace of the Ricci tensor one obtains Ricci scalar
\begin{equation} \label{eq:9}
	g^{\mu\nu}R_{\mu\nu}=R\ .
\end{equation}
Notice that they can all be obtained from the metric tensor, since the connection is given by derivatives of the metric, c.f. Eq. \eqref{eq:6}, and all these tensors are obtained from the connection.

%\par \textbf{Maybe can add a little discussion about the Bianchi identities, but for now I will wait until I figure if it is relevant to the rest of the work or not.}

%\par This is a very short summary of the mathematics of GR. It is by no means intended to be a formal introduction, but rather just a recall for the basic properties and expressions of tensors that will appear in the next sections. %Again we refer to the literature mentioned in the beginning of this chapter for a more extensive and comprehensive exposition of this topic.

\subsection{The Einstein-Hilbert action}
\par The action principle, method of minimising the an action in order to find the equations of motion, is the quickest way to introduce the Einstein equation. It is also useful in the context of AdS/CFT since the action plays an important role when it comes to computing thermodynamics and correlation functions for the dual CFT.

\par One usually applies the action principle by writing the action functional as
\begin{equation} \label{eq:10}
	S=\int d^{4}x\sqrt{-g}\mathcal{L}\ ,
\end{equation}
where $\mathcal{L}$ is, in fact, a sum of various contributions to the action, i.e. electromagnetic, gravitational, scalar, more general gauge fields, etc. The principle states that the variation of the action \eqref{eq:10}  (which is a minimum)  vanishes, and the solution to this problem are the equations of motion of the system. 

\par Let $\mathcal{L}$ in Eq. \eqref{eq:10} be
\begin{equation} \label{eq:11}
	\mathcal{L} = \mathcal{L}_{grav}+\mathcal{L}_{matter}\ ,
\end{equation}
where there first term comprises all the effects of the gravitational field in the paradigm of GR, which means that it describes how the curvature of the spacetime is modified by the second term, which is everything else.\footnote{In GR any other field that is not the metric is considered matter since it contributes to the energy momentum tensor.}

\par The gravitational part of the Lagrangian \eqref{eq:11} is given by
\begin{equation} \label{eq:12}
	\mathcal{L}_{grav}=\frac{8\pi G}{c^4}\left(R+2\Lambda\right)\ ,
\end{equation}
where $R$ is the scalar curvature, c.f. Eq. \eqref{eq:9}, and $\Lambda$ the cosmological constant. The action $S=\int d^4x \sqrt{-g}\frac{8\pi G}{c^4}\left(R+2\Lambda\right)$ is usually called Hilbert Action (or Einstein-Hilbert action) after David Hilbert who first introduced it as a way to obtain Einstein's equations. Recall that Einstein himself derived his equation using geometric arguments and the conservation of the energy-momentum tensor \cite{Einstein:1915by}.

\par Writing Eq. \eqref{eq:10} using Eqs. \eqref{eq:11} and \eqref{eq:12} one finds
\begin{equation} \label{eq:13}
	S=\int d^4x\sqrt{-g}\left[\frac{1}{2\kappa}\left(R+2\Lambda\right)+\mathcal{L}_{matter}\right]\ ,
\end{equation}
where $\frac{1}{2\kappa}=\frac{8\pi G}{c^4}$. Variation of Eq. \eqref{eq:13} with respect to the metric tensor\footnote{Variations can be taken with respect to any field appearing in the action functional, it is usually written as $\frac{\delta S}{\delta\Phi}=0$, where $\Phi$ is the field. In fact this is just a cumbersome notation, what is meant is $\delta S=\int d^4x\delta \Phi[\ldots]=0$.} leads to the Einstein's equation. Consider the general form of the variation of \eqref{eq:13}:
\begin{align}
\begin{aligned} \label{eq:14}
	\delta S&=\int d^{4}x\delta g^{\mu\nu}\left[\frac{1}{2\kappa}\frac{\delta\left(\sqrt{-g}R\right)}{\delta g^{\mu\nu}}+\frac{\delta\left(\sqrt{-g}\mathcal{L}_{matter}\right)}{\delta g^{\mu\nu}}\right]\\
	&=\int d^{4}x\delta g^{\mu\nu}\left[\frac{1}{2\kappa}\left(R\frac{\delta\sqrt{-g}}{\delta g^{\mu\nu}}+\sqrt{-g}\frac{\delta R}{\delta g^{\mu\nu}}\right)+\frac{\delta\left(\sqrt{-g}\mathcal{L}_{matter}\right)}{\delta g^{\mu\nu}}\right]\\
	&=\int d^{4}x\delta g^{\mu\nu}\sqrt{-g}\left[\frac{1}{2\kappa}\left(\frac{R}{\sqrt{-g}}\frac{\delta\sqrt{-g}}{\delta g^{\mu\nu}}+\frac{\delta R}{\delta g^{\mu\nu}}\right)+\frac{1}{\sqrt{-g}}\frac{\delta\left(\sqrt{-g}\mathcal{L}_{matter}\right)}{\delta g^{\mu\nu}}\right]
\end{aligned}
\end{align}
The second term inside the square brackets is defined as the energy momentum tensor
\begin{equation} \label{eq:15}
	T_{\mu\nu}=-\frac{2}{\sqrt{-g}}\frac{\delta\left(\sqrt{-g}\mathcal{L}_{matter}\right)}{\delta g^{\mu\nu}}\ .
\end{equation}
Since this variarion must hold for arbitrary $\delta g^{\mu\nu}$ the geometric part of Einstein's equation is obtained from the term:
\begin{equation} \label{eq:16}
\frac{R}{\sqrt{-g}}\frac{\delta\sqrt{-g}}{\delta g^{\mu\nu}}+\frac{\delta R}{\delta g^{\mu\nu}}= G_{\mu\nu}
\end{equation}
as will be shown.

\par Variation of the determinant requires using the following identity
\begin{equation}\label{eq:17}
	\ln\left(\det M\right)=\text{Tr}\left(\ln M\right)\ ,
\end{equation}
which applies to any matrix $M$.\footnote{$\ln M$ is defined by $\exp\ln M$.} Varying this identity leads to
\begin{align}
	\begin{aligned}	\label{eq:18}
	\delta\ln\left(\det M\right)&=\delta\text{Tr}\left(\ln M\right) \\
	\frac{1}{\det M}\delta M&=\text{Tr}\left(M^{-1}\delta M\right)
	\end{aligned}
\end{align}
Now let $\det M=\det g_{\mu\nu}=g$\, thus
\begin{align} \label{eq:19}
	\delta g&=gg^{\mu\nu}\delta g_{\mu\nu}\ .
\end{align}
Finally, putting all the pieces together to write the variation of $\sqrt{-g}$:
\begin{align}
	\begin{aligned} \label{eq:20}
	\delta\sqrt{-g}&=-\frac{1}{2\sqrt{-g}}\delta g\\
	&=-\frac{g}{2\sqrt{-g}}g^{\mu\nu}\delta g_{\mu\nu}\\
	&=\frac{g}{2\sqrt{-g}}g_{\mu\nu}\delta g^{\mu\nu}\\
	&=-\frac{\sqrt{-g}}{2}g_{\mu\nu}\delta g^{\mu\nu}
	\end{aligned}
\end{align}
Notice that the sign change from the second to third line occurs because $\delta\left(g^{\mu\nu}g_{\mu\nu}\right)=\delta\left[\text{Tr}(\text{Id})\right]=0\implies g_{\mu\nu}\delta g^{\mu\nu}+g^{\mu\nu}\delta g_{\mu\nu}=0$.

\par The second term on the left hand side of Eq. \eqref{eq:16} requires to look back on the definition of the scalar curvature (c.f. Eq. \eqref{eq:9}) as the trace of the contraction of the Riemann tensor. Thus, by varying the Riemann tensor, which according to Eq. \eqref{eq:7} is
\begin{equation} \label{eq:21}
	\delta R_{\text{ }\theta\mu\nu}^{\lambda}=\partial_{\mu}\delta\Gamma_{\nu\theta}^{\lambda}-\partial_{\nu}\delta\Gamma_{\mu\theta}^{\lambda}+\Gamma_{\mu\alpha}^{\lambda}\delta\Gamma_{\nu\theta}^{\alpha}+\Gamma_{\mu\alpha}^{\lambda}\delta\Gamma_{\nu\theta}^{\alpha}-\Gamma_{\nu\alpha}^{\lambda}\delta\Gamma_{\mu\theta}^{\alpha}-\Gamma_{\mu\theta}^{\alpha}\delta\Gamma_{\nu\alpha}^{\lambda}+\Gamma_{\nu\theta}^{\alpha}\delta\Gamma_{\mu\alpha}^{\lambda}\ .
\end{equation}
The variation of the connection is defined by $\Gamma_{\mu\nu}^{\lambda}\mapsto\Gamma_{\mu\nu}^{\lambda}+\delta\Gamma_{\mu\nu}^{\lambda}$, i.e. $\delta\Gamma_{\mu\nu}^{\lambda}$ is the difference between two connections, therefore it is a tensor. This fact allows one to take the covariant derivative $\nabla_{\alpha}\delta\Gamma_{\mu\nu}^{\lambda}$:
\begin{equation}\label{eq:22}
	\nabla_{\mu}\delta\Gamma_{\nu\theta}^{\lambda}=\partial_{\mu}\delta\Gamma_{\mu\theta}^{\lambda}+\Gamma_{\mu\alpha}^{\lambda}\delta\Gamma_{\nu\theta}^{\alpha}-\Gamma_{\mu\nu}^{\alpha}\delta\Gamma_{\alpha\theta}^{\lambda}-\Gamma_{\mu\theta}^{\alpha}\delta\Gamma_{\nu\alpha}^{\lambda}\ ,
\end{equation}
and similarly for $\nabla_{\nu}\delta\Gamma_{\mu\theta}^{\lambda}$. After a little algebra one sees that Eq. \eqref{eq:21} is equivalent to
\begin{equation}\label{eq:23}
	\delta R_{\text{ }\theta\mu\nu}^{\lambda}=\nabla_{\mu}\delta\Gamma_{\nu\theta}^{\lambda}-\nabla_{\nu}\delta\Gamma_{\mu\theta}^{\lambda}\ .
\end{equation}
Contraction of Eq. \eqref{eq:23} gives the variation of Ricci tensor
\begin{equation}\label{eq:24}
	\delta R_{\theta\nu}=\delta R_{\text{ }\theta\mu\nu}^{\mu}=\nabla_{\mu}\delta\Gamma_{\nu\theta}^{\mu}-\nabla_{\nu}\delta\Gamma_{\mu\theta}^{\mu}\ .
\end{equation}
Multiplying by the inverse metric the variation of scalar curvature is obtained:
\begin{align}
	\begin{aligned}\label{eq:25}
	\delta R=g^{\mu\nu}\delta R_{\mu\nu}&=g^{\mu\nu}\left(\nabla_{\alpha}\delta\Gamma_{\mu\nu}^{\alpha}-\nabla_{\nu}\delta\Gamma_{\mu\alpha}^{\alpha}\right)\\
	&=\nabla_{\alpha}g^{\mu\nu}\delta\Gamma_{\mu\nu}^{\alpha}-\nabla_{\nu}g^{\mu\nu}\delta\Gamma_{\mu\alpha}^{\alpha}\\
	&=\nabla_{\alpha}\left(g^{\mu\nu}\delta\Gamma_{\mu\nu}^{\alpha}-g^{\mu\alpha}\delta\Gamma_{\mu\nu}^{\nu}\right)
	\end{aligned}
\end{align}
where it is shown that this particular variation can be written as a single covariant derivative, which upon multiplication by $\sqrt{-g}$ becomes a total derivative, so by Stokes theorem the integral of this term vanishes:
\begin{equation} \label{eq:26}
	\int d^{4}x\sqrt{-g}\nabla_{\alpha}\left(g^{\mu\nu}\delta\Gamma_{\mu\nu}^{\alpha}-g^{\mu\alpha}\delta\Gamma_{\mu\nu}^{\nu}\right)=0\ .
\end{equation}
Finally, notice that from the definition of scalar curvature, Eq. \eqref{eq:9}:
\begin{equation}\label{eq:27}
	\delta\left(g^{\mu\nu}R_{\mu\nu}\right)=R_{\mu\nu}\delta g^{\mu\nu}-g^{\mu\nu}\delta R_{\mu\nu}\ ,
\end{equation}
from Eq. \eqref{eq:26} it is seen that the second term vanishes upon integration, so the action in Eq. \eqref{eq:14} becomes
\begin{equation} \label{eq:28}
	\delta S=\int d^{4}x\delta g^{\mu\nu}\sqrt{-g}\left[\frac{1}{2\kappa}\left(-\frac{R}{2}g_{\mu\nu}+R_{\mu\nu}\right)-\frac{1}{2}T_{\mu\nu}\right]\ ,
\end{equation}
where Eqs. \eqref{eq:15}, \eqref{eq:20} and \eqref{eq:27} were used. The term in the square brackets are clearly Einstein's equations
\begin{equation} \label{eq:29}
	R_{\mu\nu}-\frac{R}{2}g_{\mu\nu}=\kappa T_{\mu\nu}\ .
\end{equation}

\par As a final remark for this session it must be said that the cosmological constant present in Eq. \eqref{eq:13} was not considered but it can be easily seen that its contribution to the Einstein's equation can be derived from Eq. \eqref{eq:20}, since that is the only variation contributing. The Einstein's equation including the cosmological constant $\Lambda$ are
\begin{equation} \label{eq:30}
	R_{\mu\nu}-\frac{R}{2}g_{\mu\nu}+\Lambda g_{\mu\nu}=\kappa T_{\mu\nu}\ .
\end{equation}
The cosmological constant allows for solutions with positive and negative constant curvature in vacuum, which are of great importance in this work. In the next section some solutions to Einstein's equation, with and without cosmological constant, are discussed and, in next chapters, the importance of solution in the presence of cosmological constant will become clear.

\section{Some solutions of Einstein's equations} \label{sec:2}
\par In this section solutions of interest to the development of this work are presented and discussed. By looking at Eq. \eqref{eq:30} we can see that the Einstein's equations are a set of 10 partial differential equations for the metric components. If one were to write down all the equations in its most general form and try to solve it, would quickly realise that such task is nearly impossible. For that reason restrictions are made in order to obtain solutions, these restrictions usually are imposed as symmetries of the space-time, which greatly simplify the left hand side of Eq. \eqref{eq:30}.

\par Three solutions are discussed here: anti-de Sitter space-time, Schwarzschild and Reissner-Nordstr\"om black holes. Of course there are other solutions, but these are of no relevance to this work. The reason these three solutions are presented here will become clear when the holographic correspondence is introduced, in future chapters.

\subsection{Anti-de Sitter space-time} \label{sec:2.1}
\par There is a class of solutions to Einstein's equations called maximally symmetric spaces. Long story short, these space-times have all possible symmetries allowed and it can be shown that it depends on the scalar curvature. For a $D-$dimensional manifold there are $\frac{1}{2}D(D+1)$ possible symmetries, which are translations and rotations along all the axis (recall that when the space-time has lorentzian signature some rotations are actually boosts, but this does not change the counting of symmetries). For such a manifold the curvature must be the same everywhere, which means that the Riemann tensor doesn't change at all, regardless of symmetry transformations done to its components. In fact there are only three tensors that are invariant under these conditions: the Kronecker delta, Levi-Civita tensor (totally anti-symmetric tensor) and the metric tensor. Thus the Riemann curvature tensor must be, at most, a combination of these three in such circumstance. Analysing the symmetries of the Riemann tensor it is not hard to figure out that there is only one combination:
\begin{equation}\label{eq:31}
	R_{\mu\nu\lambda\theta}=k\left(g_{\mu\lambda}g_{\nu\theta}-g_{\mu\theta}g_{\nu\lambda}\right)\ ,
\end{equation}
where $k$ is determined by contracting the expression twice with the metric tensor. In doing that one obtains
\begin{equation}\label{eq:32}
	k=\frac{R}{D\left(D-1\right)}\ .
\end{equation}

\par Eqs. \eqref{eq:31} and \eqref{eq:32} show that maximally symmetric spaces are basically described by the scalar curvature and, since it is the same everywhere, there are only three possibilities: positive, negative and zero. For vanishing scalar curvature it is obvious that the Riemann tensor will vanish as well (c.f.  Eq. \eqref{eq:31}), and that is Minkowski space-time, the space-time of Special Relativity. For positive and negative values they produce the solutions called de Sitter and anti-de Sitter space-times, respectively. This is where the cosmological constant, $\Lambda$ in Eq. \eqref{eq:30}, plays an important role. Consider Einstein's equation in vacuum, i.e. $T_{\mu\nu}=0$ and take its trace, from Eq. \eqref{eq:30}:
\begin{equation} \label{eq:33}
	R=4\Lambda\ ,
\end{equation}
thus one sees that if the cosmological constant is absent the only possibility for the scalar curvature is actually zero. Also notice that the sign of the cosmological constant determines the sign of the scalar curvature. In the reminder of this subsection the solution for negative cosmological constant is treated, hence negative scalar curvature, which is called the anti-de Sitter space-time.

\par It is usual to rename the constant $k$ in Eq. \eqref{eq:32} as
\begin{equation} \label{eq:34}
	k=\frac{1}{L^2}\ ,
\end{equation}
where $L$ is called radius of curvature, thus
\begin{align}\label{eq:35}
	R=\frac{D\left(D-1\right)}{L^{2}}\text{, }&\Lambda=-\frac{D\left(D-1\right)}{4L^{2}}\ .
\end{align}

\par The explicit expression for the metric is obtained by embedding the solution in a higher dimensional space time, let its dimension be $N=D+1$, and the metric given by the following expression in coordinates $\left\{ \xi^{0},\ldots,\xi^{D}\right\}$
\begin{equation} \label{eq:36}
	ds^{2}=-\left(d\xi^{0}\right)^{2}-\left(d\xi^{1}\right)^{2}+\left(d\xi^{2}\right)^{2}+\left(d\xi^{3}\right)^{2}+\ldots+\left(d\xi^{n}\right)^{2}\ ,
\end{equation}
i.e. $\mathbb{R}^{(n-1,2)}$. Then AdS space-time is defined by the constraint
\begin{equation}\label{eq:37}
	\xi_{\mu}\xi^{\mu}=-\left(\xi^{0}\right)^{2}-\left(\xi^{1}\right)^{2}+\left(\xi^{2}\right)^{2}+\ldots+\left(\xi^{n}\right)^{2}=-L^{2}\ .
\end{equation}
This is a hyperboloid. Considering the case for $D=4$ one parametrization is given by
\begin{align}
	\begin{aligned}\label{eq:38}
	\xi^{0}=L\sin\left(\frac{t}{L}\right)\cosh\left(\frac{r}{L}\right),\ \ \ \
	\xi^{1}=L\cos\left(\frac{t}{L}\right)\cosh\left(\frac{r}{L}\right),\ \ \ \
	\vec{\xi}=L\sinh\left(\frac{r}{L}\right)\vec{n},
	\end{aligned}
\end{align}
where $\vec{\xi}=\left(\xi^2,\xi^3,\xi^4\right)$ and $\vec{n}=\left(\sin\theta\cos\phi,\sin\theta\sin\phi,\cos\theta\right)$, so the metric is
\begin{equation}\label{eq:39}
	ds^{2}=L^{2}\left(-\cosh^{2}\left(\frac{R}{L}\right)dt^{2}+dr^{2}+\sinh^2\left(\frac{r}{L}\right)d\Omega_{2}^{2}\right)\ .
\end{equation}
Notice that $t=const.$ is the metric of a hyperbolic space (in fact it \textit{is} the space called $H^3$ by mathematicians). Two things that should be remarked about Eq. \eqref{eq:39} are: i) it has a singularity along $r=0$, ii) its time coordinate is periodic. Both of these problems are due to the choice of coordinates in Eq. \eqref{eq:38}, in fact, these coordinates are not of much use and another coordinate system is more suitable to describe AdS space-time.

\par Define the coordinates $\left\{ t,r,x,y\right\} =\left\{ t,r,\vec{x}\right\}$ in the following way
\begin{align}
	\begin{aligned} \label{eq:40}
	\xi^{0}=\frac{L}{2r}\left(1+\frac{r^{2}}{L^{4}}\left(L^{2}+\vec{x}^{2}-t^{2}\right)\right), \ \ \ \
	\xi^{1}=\frac{r}{L}t,\ \ \ \
	\xi^{i}=\frac{r}{L}x^{i},\ \ \ \
	\xi^{D+1}=\frac{L}{2r}\left(1-\frac{r^{2}}{L^{4}}\left(L^{2}+\vec{x}^{2}-t^{2}\right)\right),
	\end{aligned}
\end{align} 
in these coordinates Eq. \eqref{eq:36} becomes
\begin{equation}\label{eq:41}
	ds^{2}=-\frac{r^{2}}{L^{2}}dt^{2}+\frac{L^{2}}{r^{2}}dr^{2}+\frac{r^{2}}{L^{2}}d\vec{x^{2}}\ .
\end{equation}
This is the AdS space-time in the so called Poincaré Coordinates, it is the most commonly used coordinate system in holography. Notice that in these coordinates $-\infty<t<\infty$, $r>0$. The singularity is located at the point $r=0$, but now it can be seen to be a Killing horizon. Also $r\rightarrow\infty$ approaches the boundary of AdS space-time, sometimes called the conformal boundary, for it is in fact Minkowski space-time with conformal factor $r/L$.

\par Now, by defining $u=r/L$ Eq. \eqref{eq:41} reads
\begin{equation}\label{eq:42}
	ds^{2}=L^{2}\left(\frac{du^{2}}{u^{2}}+u^{2}dx_{\mu}dx^{\mu}\right)\ ,
\end{equation}
where $dx_{\mu}dx^{\mu}=-dt^{2}+d\vec{x}^{2}$. Further, defining $z=1/u$, Eq. \eqref{eq:42} is cast in the following form
\begin{equation} \label{eq:43}
	ds^{2}=\frac{L^{2}}{z^{2}}\left(dz^{2}+dx_{\mu}dx^{\mu}\right)\ .
\end{equation}
All forms of AdS space-time metric, Eqs. \eqref{eq:41}-\eqref{eq:43}, exhibit the same properties mentioned below Eq. \eqref{eq:41}, it is just a matter of convenience using one or another by the simple transformation that leads from one to the other.

\subsection{Black hole solutions}
\par One of the greatest achievements of General Relativity is unveiling what are called black holes. There are evidences that speculations regarding similar object have been made before the GR theory came to public, for instance John Michell and P. S. Laplace \cite{2009JAHH...12...90M} considered the existence of such objects, it was only a matter of speculation, since the theories of relativity (both special and general) are fundamental to comprehend what black holes really are and give a satisfactory description.

\par In this section only static solutions of black holes are considered, this means that, in some sense, the black holes described are stable and do not evolve in any sense\footnote{Technically a static space-time has a time like Killing vector that is orthogonal to a family of space like hyper surfaces, this means that the metric tensor can always be cast in a form such that it is independent of the time coordinate. As opposed to this kind of solution there are stationary solutions, in which case the Killing vector is only locally orthogonal to the space like hyper surfaces. Turns out that in this case the metric will have dependence on the time coordinate.}. This also means that one is not interested in the formation of such structure, thus assuming the black hole was formed by some previous process and is looked at once stability is reached.

\subsubsection*{Schwarzschild black hole}
\par The first black hole solution we will consider is actually the first solution published after GR came to public \cite{Schwarzschild:1916uq}. It is one of the simplest solutions there is, and much can be learnt from it. Consider a spherically symmetric space-time, where the cosmological constant is zero and there is no matter in the region of interest. By vacuum it is meant $T_{\mu\nu}=0$, so Einstein's equation, c.f. Eq. \eqref{eq:30}, reads
\begin{equation}\label{eq:44}
	R_{\mu\nu}-\frac{1}{2}Rg_{\mu\nu}=0\ .
\end{equation}
From Eq. \eqref{eq:44} one notices immediately that the scalar curvature vanishes, taking the trace of Eq. \eqref{eq:44}:
\begin{align}
	\begin{aligned}\label{eq:45}
	g^{\mu\nu}\left(R_{\mu\nu}-\frac{1}{2}Rg_{\mu\nu}\right)=R-2R=R=0\\
	\end{aligned}
\end{align}
In fact, Einstein's equations for this problem are
\begin{equation}\label{eq:46}
	R_{\mu\nu}=0\ .
\end{equation}

\par To solve Eqs. \eqref{eq:46}, the following ansatz is a suitable one
\begin{equation}\label{eq:47}
	ds^{2}=-e^{2a\left(r\right)}dt^{2}+e^{2b\left(r\right)}dr^{2}+r^{2}d\Omega^{2}\ .
\end{equation}
The exponentials are used mainly to keep the metric with the same signature in the end. Notice that the ansatz \eqref{eq:47} is a generalization of Minkowski flat space-time, where the element $d\Omega=d\theta^2+\sin^2\theta d\phi$ is kept the same to preserve spherical symmetry. Given the ansatz it is a matter of computation to calculate the non-vanishing components of Ricci tensor and solving the differential equations. If one is interested in the full system of equations, it can be found in \cite{Carroll:2004st}, where all the tensor components are displayed, here only relevant parts of the calculations are going to mentioned.

\par Plugging Eq. \eqref{eq:47} into Eq. \eqref{eq:46} one is faced by 4 ordinary differential equations, since the only variable in the problem is the radial coordinate $r$. In fact only three of these equations are independent, since it is easy to see that $R_{\theta\theta}=R_{\phi\phi}\sin^2\theta$, thus there are three equations to determine two functions: $a(r)$ and $b(r)$. Combining equations $R_{tt}+R_{rr}=0$, the important condition is found:
\begin{equation}\label{eq:48}
	a(r)=-b(r)+const.\ ,
\end{equation}
where the constant can be set to zero by shifting the time coordinate $t\rightarrow e^{-const.}t$. Then the equation $R_{\theta\theta}=0$ gives
\begin{equation}\label{eq:49}
	\frac{d}{dr}\left(re^{2a\left(r\right)}\right)=1\ ,
\end{equation}
which has solution
\begin{equation}\label{eq:50}
	e^{2a}=1-\frac{R_{S}}{r}\ .
\end{equation}
From Eqs. \eqref{eq:48} and \eqref{eq:50} the celebrated Schwarzschild metric for a static black hole is obtained
\begin{equation}\label{eq:51}
	ds^{2}=-\left(1-\frac{R_{S}}{r}\right)dt^{2}+\left(1-\frac{R_{S}}{r}\right)^{-1}dr^{2}+r^{2}d\Omega^{2}\ .
\end{equation}
The constant $R_S$ is called the Schwarzschild radius, and it can be shown that $R_S=2M$ with $M$ being the mass of the black hole. This identification is made by taking the low energy limit of GR \cite{Carroll:2004st,Wald:1984rg}. The limit $r\rightarrow\infty$ leads Eq. \eqref{eq:51} to the usual Minkowski space-time in spherical coordinates, as it is easily seen.

\par One question that should be addressed is: If the Schwarzschild black hole is a solution for Einstein's equations in vacuum how does the mass of the black hole appears in the solution? Or even, what is the black hole after all, since no matter terms were considered in the lagrangian at all? In fact, matter is absent in our solution, but the fact that we are describing the outer region of the black hole with the particular solution \eqref{eq:51} does not mean there is no matter content. Indeed there is a point like, massive, particle that produces such curvature and, for all effects, this is sufficient since we are not describing the massive object itself, but just the space-time surrounding it.

\par Moreover, the surface $R=R_S$ is what is called an event horizon. This surface has such a strong gravitational acceleration that its escape velocity is equal to the speed of light, meaning that everything at $R_S$ and nearer cannot escape. On first glance $R_S$ may seem a weird spot since $g_{tt}\rightarrow0$ and $g_{rr}\rightarrow\infty$, but this is only a problem of the coordinate system. In this work other coordinate systems won't be covered, so we refer to \cite{Misner:1974qy} for a wider discussion on this topic. One way to realise that there is no problem with the surface $r=R_S$ is by evaluating the so called Kretschmann scalar $K=R^{\mu\nu\lambda\rho}R_{\mu\nu\lambda\rho}$ at this point, since $R=0$ we have to rely on other geometric scalar. Once $K$ is evaluated one can see that the only singular point in the whole space-time \eqref{eq:51} is $r=0$, i.e. where the mass is localized. This point is really a singularity and there is nothing we can do to avoid it, like it or not - think of it like the divergence found when approaching the charge in the electric field of a point-like charge in Coulomb's law, or the gravitational acceleration of a point like mass using Newton's inverse square law.

\par The existence of the event horizon is what gives the name to black holes. In technical terms the event horizon is a null surface, typically in this regions there are changes in the causal structure of the space-time itself \cite{Wald:1984rg}. In the simple case of Schwarzschild black hole it is only a function of the mass of the object but, as will be seen in the next chapter, it can depend on other properties of the black hole, such as electric charge and angular momentum. Due to the no hair theorem these are the only properties that determine a black hole \cite{Hawking:1973uf}.

\subsubsection*{Reissner-Nordström black hole} \label{GR:RNsol}

\par In a similar fashion to the previous black hole solution, consider a spherically symmetric space-time where, at the origin, we place a point like particle with mass $M$ and charge $Q$. So, besides from the addition of the electric charge, this is the Schwarzschild black hole and thus one condition is that once $Q\rightarrow0$, Eq. \eqref{eq:51} must be recovered.

\par Since the electric charge is present this space-time is no longer vacuum. Although no material content is found in the region of interest, that is outside the event horizon, we still have the presence of the electric field. For this reason the Reissner-Nordström space-time is referred to as the electro-vacuum solution \cite{1916AnP...355..106R,1918KNAB...20.1238N}. A matter term must be added to the action to account for this electric field, it is the free part of the Maxwell lagrangian
\begin{equation} \label{eq:52}
	\mathcal{L}_{matter}=-\frac{1}{4}F_{\alpha\beta}F^{\alpha\beta}\ ,
\end{equation}
where $F_{\mu\nu}$ is the Maxwell tensor, defined from the gauge potential $A_{\mu}$ by $F_{\mu\nu}=2\partial_{[\mu}A_{\nu ]}$. The energy momentum tensor, c.f. Eq. \eqref{eq:15}, can be written as
\begin{equation}\label{eq:53}
	T_{\mu\nu}=-2\frac{\delta\mathcal{L}_{matter}}{\delta g^{\mu\nu}}+g_{\mu\nu}\mathcal{L}_{matter}\ ,
\end{equation}
by the product rule and using Eq. \eqref{eq:20}. The variation of Eq. \eqref{eq:52} is
\begin{align}
	\begin{aligned}
	-\frac{1}{4}\frac{\delta}{\delta g^{\mu\nu}}\left(F_{\alpha\beta}F^{\alpha\beta}\right)&=-\frac{1}{4}\frac{\delta}{\delta g^{\mu\nu}}\left(g^{\lambda\alpha}g^{\rho\beta}F_{\alpha\beta}F_{\lambda\rho}\right)\\
	&=-\frac{1}{4}F_{\alpha\beta}F_{\lambda\rho}\left[g^{\rho\beta}\frac{\delta}{\delta g^{\mu\nu}}g^{\lambda\alpha}+g^{\lambda\alpha}\frac{\delta}{\delta g^{\mu\nu}}g^{\rho\beta}\right]\\
	&=-\frac{1}{4}F_{\alpha\beta}F_{\lambda\rho}\left[\frac{1}{2}g^{\rho\beta}\left(\delta_{\mu}^{\lambda}\delta_{\nu}^{\alpha}+\delta_{\nu}^{\lambda}\delta_{\mu}^{\alpha}\right)+\frac{1}{2}g^{\lambda\alpha}\left(\delta_{\mu}^{\rho}\delta_{\nu}^{\beta}+\delta_{\nu}^{\rho}\delta_{\mu}^{\beta}\right)\right]\\
	&=-\frac{1}{4}\left[\frac{1}{2}\left(F_{\nu\beta}F_{\mu}^{\text{ }\beta}+F_{\mu\beta}F_{\nu}^{\text{ }\beta}\right)+\frac{1}{2}\left(F_{\alpha\nu}F_{\text{ }\mu}^{\alpha}+F_{\alpha\mu}F_{\text{ }\nu}^{\alpha}\right)\right]\\
	&=-\frac{1}{2}F_{\mu\alpha}F_{\nu}^{\text{ }\alpha}
	\end{aligned}
\end{align}
So Eq. \eqref{eq:53} gives the energy momentum tensor of the electromagnetic field
\begin{equation} \label{eq:55}
	T_{\mu\nu}=F_{\mu\alpha}F_{\nu}^{\text{ }\alpha}-\frac{1}{4}g_{\mu\nu}F_{\alpha\beta}F^{\alpha\beta}\ .
\end{equation}

\par Remember that the matter content also has its equations of motion, in this case variation of Eq. \eqref{eq:52} with respect to the gauge potential $A_{\mu}$ simply gives the homogeneous Maxwell's equations
\begin{equation} \label{eq:56}
	\partial_{\mu}\left(\sqrt{-g}F^{\mu\nu}\right)=0\ .
\end{equation}
The problem is then formulated: the Reissner-Nordström black hole is the solution of the system of Einstein-Maxwell's equations,Eqs. \eqref{eq:29}, \eqref{eq:56}, with energy momentum tensor given by Eq. \eqref{eq:55}.

\par The same ansatz used in to solve for Schwarzschild will be used here, c.f. Eq. \eqref{eq:47}, since that ansatz was a general one for a static spherically symmetric space-time. And noticing that
\begin{align}
	\begin{aligned}\label{eq:57}
	g^{\mu\nu}T_{\mu\nu}&=g^{\mu\nu}\left(F_{\mu\alpha}F_{\nu}^{\text{ }\alpha}-\frac{1}{4}g_{\mu\nu}F_{\alpha\beta}F^{\alpha\beta}\right)=F_{\mu\alpha}F^{\mu\alpha}-F_{\alpha\beta}F^{\alpha\beta}=0
	\end{aligned}
\end{align}
The computation in Eq. \eqref{eq:45} is valid in this context as well. As for the components of $F_{\mu\nu}$, and consequently $T_{\mu\nu}$, we have only $F_{tr}\neq0$ which is the radial component of the electric field. For a point like charge that is not moving this is the only non zero component.\footnote{If one wishes to generalize there is the option of including magnetic monopoles, which will generate a radial magnetic field. Turns out that the solution will be exactly the same, except that the charge we will find would be the sum of the magnetic and electric charge.} So, let
\begin{equation} \label{eq:58}
	E_r=F_{tr}=f(r)\ ,
\end{equation}
we have not allowed a time dependence in this function, although in a more general case it should be considered. Turns out that one of the components of Maxwell's equation, together with the fact that space-time is static, leads to an independence of time \cite{Carroll:2004st}.

\par For the sake of lengthiness the full calculations are not carried over, one can find it amongst the literature referred to in the begging of this chapter. The components $T_{tt}$ and $T_{rr}$ are equal and have opposite sign, thus the combination $R_{tt}+R_{rr}=0$ holds and the result, Eq. \eqref{eq:48}, is obtained. It is now possible to solve the Maxwell equation for the electric field, the $t$-component of Eq. \eqref{eq:56} will be, after all substitutions
\begin{align}
\begin{aligned}\label{eq:59}
\partial_{r}\left(r^{2}F^{rt}\right)=\partial_{r}\left(r^{2}f\right)=0
\implies f\left(r\right)=\frac{const.}{r^{2}}
\end{aligned}
\end{align}
The constant is identified with the electric charge, $Q$, requiring that this assumes the form of Coulomb's law of electrostatics.

\par Now there is only the $\theta\theta$-component of Einstein's equations to be solved, the differential equation is slightly different from Eq. \eqref{eq:49}, in fact, it reads
\begin{equation}\label{eq:60}
	\frac{d}{dr}\left(re^{2a\left(r\right)}\right)=1-\frac{Q^{2}}{r^{2}}\ ,
\end{equation}
and the solution is
\begin{equation}
	e^{2a\left(r\right)}=1-\frac{R_{S}}{r}+\frac{Q^{2}}{r^{2}}\ .
\end{equation}
From our ansatz and considerations made here we find the Reissner-Nortström metric
\begin{equation}\label{eq:62}
	ds^{2}=-\left(1-\frac{R_{S}}{r}+\frac{Q^{2}}{r^{2}}\right)dt^{2}+\left(1-\frac{R_{S}}{r}+\frac{Q^{2}}{r^{2}}\right)^{-1}dr^{2}+r^{2}d\Omega^{2}\ .
\end{equation}

\par Differently from Schwarzschild space-time we can readily see that there are 2 singular surfaces for the $r$ coordinate, these are usually denoted by $r_{\pm}$, and one can verify that its dependent on the mass and charge of the black hole:
\begin{equation}\label{eq:63}
	r_{\pm}=M\pm\sqrt{M^{2}-Q^{2}}\ .
\end{equation}
These two are in fact null hypersurfaces, meaning they are indeed event horizons of the space-time. Again, the fact that components of the metric vanish or diverge at these values has to do with the coordinate system being used to describe the space-time, the only point that shows a divergence that cannot be avoided is $r=0$, which can be seen by evaluation of curvature scalars such as the Kretschmann scalar.

\par One interesting feature of the space-time given by Eq. \eqref{eq:62} is that one can imagine a black hole which all its mass is due to electric charge, $Q$. In such case $r_{+}=r_-=r_0$ have the same value $r_0=Q$. Such a black hole is called extreme black hole and before AdS/CFT not much attention has been given to it, besides the fact that it is an interesting curiosity, since for practical (astrophysical) purposes it is irrelevant since in interstellar media such an object would quickly acquire zero net charge. More will be said about the extreme Reissner-Nordström black hole in future chapters.

\section{Thermodynamics of black holes}\label{sec:3}

\par In the late 60's and during the 70's it was found that black holes obey a set of laws that resembles the laws of thermodynamics, the works of Carter, Bekenstein, Hawking and many others \cite{Bardeen:1973gs, Bekenstein:1973ur, Hawking:1974rv} are seminal references to the topic which lives to this day, and in fact constitutes a research area on its own. It all started as an analogy, originated from the similarity between equations obtained for black holes and the already knows laws of thermodynamics, but far from stopping at this point, it is actually shown formally that the laws of black hole mechanics hold in their own and the term thermodynamics of black holes is used merely as terminology.

\par Here the laws of black hole mechanics are stated and some of its most important features are highlighted, since the subject is very technical and would demand the introduction of a large mathematical machinery we refer to \cite{Hawking:1973uf, Wald:1995yp} for a complete discussion.

\par The zeroth law of thermodynamics defines temperature using equilibrium states. For black holes the analogue of an equilibrium state is a stationary space-time, which is the faith of a black hole.\footnote{The black holes encountered in \ref{sec:2} are static space-times, which is a further specialisation of stationary solutions of Einstein's equations.} It can be shown that a quantity called surface gravity is a constant everywhere at the event horizon of a stationary black hole \cite{Wald:1995yp}, when measured by an observer at asymptotic infinity. It is defined in pure geometrical terms as \cite{Wald:1984rg}
\begin{equation}\label{eq:64}
	\kappa^{2}=\lim_{r\rightarrow r_{0}}\left[\frac{\left(\xi^{\mu}\nabla_{\mu}\xi^{\lambda}\right)\left(\xi^{\nu}\nabla_{\nu}\xi_{\lambda}\right)}{\xi^{\rho}\xi_{\rho}}\right]\ ,
\end{equation}
where $\xi$ is the time like Killing vector, and we are considering the case for a static space-time - for a more general, stationary solution, the expression is similar but the Killing vector is a linear combination -. For static space-times the Killing vector is simply $\xi_{\mu}=\partial_{t}$.\footnote{It is worth mentioning that \eqref{eq:64} will only work when the coordinates are regular at the horizon, otherwise it will lead to a meaningless expression.}

\par Identifying Eq. \eqref{eq:64} with the actual surface gravity requires some effort, the proof is found in \cite{Wald:1984rg}, after the calculations it can be verified that
\begin{equation}
	\kappa=\lim_{r\rightarrow r_{0}}(Va)\ ,
\end{equation}
where $V$ is the redshift factor and $a$ the magnitude of the four acceleration. Essentially the surface gravity measures the force necessary to keep a particle from falling into the event horizon, such force is measured by an observer at infinity. The formal relation between the surface gravity and temperature is given by
\begin{equation}\label{eq:66}
	T=\frac{\kappa}{2\pi}\ ,
\end{equation}
it was derived first by Hawking \cite{Hawking:1974rv} in his work where he also introduced the so called Hawking radiation, which is the cornerstone for the development of thermodynamics of black holes - it was this work that started to establish the laws of black hole mechanics, before that it was considered an analogy with classical thermodynamic equations.

\par Next consider the most general black hole there can be, it is called Kerr-Newman black hole \cite{Newman:1965my}. It was not covered in these chapter, and will not be covered anywhere in this work, but it is the simplest way to obtain the fist law of black hole mechanics (the analogue of first law of thermodynamics for black holes). The Kerr-Newman black hole has all the properties allowed by no-hair theorem: mass, charge and angular momentum. It is a stationary and axi-symmetric space-time, and its derivation as well as properties go far beyond those of Schwarzschild and Reissner-Nordstr\"om.

\par In \cite{Smarr:1973zz} it is shown that the surface area of the horizon of Kerr-Newman black hole is given by the following
\begin{equation}\label{eq:67}
	A=4\pi\left[2M^{2}-Q^{2}+2M^{2}\left(1-\frac{Q^{2}}{M^{2}}-\frac{J^{2}}{M^{4}}\right)^{1/2}\right]\ ,
\end{equation}
where $J$ is the angular momentum. In Eq. \eqref{eq:67} it is considered that $Q^2<M^2$ and $J^2<M^4$. From Eq. \eqref{eq:67} one can derive the following relation
\begin{equation}\label{eq:68}
	dM=\frac{1}{8\pi}\kappa dA+\Omega dJ+\Phi dQ\ ,
\end{equation}
where $\frac{1}{8\pi}\kappa=\frac{\partial M}{\partial A}, \Omega=\frac{\partial J}{\partial A}$, etc.  Eq. \eqref{eq:68} is called the first law of black hole mechanics, for it resembles the first law of thermodynamics. This law plays a crucial role in proving that Kerr-Newman is, in fact, the only black hole that can exist in an asymptotically flat space-time, governed by Einstein's equations \cite{Hawking:1973uf, Wald:1993ki}. Moreover, it is important in the study of matter accretion in black holes and galaxies, which is subject of astrophysics \cite{Raine:2005bs}.

\par The first term in Eq. \eqref{eq:68} gives a hint for the second law of black hole mechanics. Remember that $dE=TdS+\ldots$ is the first term of the first law of thermodynamics. One would be inclined to write $\kappa dA\sim TdS$, and it is actually correct to identify the entropy with the area of the black hole.  In fact the horizon area has a similar property to entropy, which is: it can only increase. I can be shown \cite{Wald:1995yp} that for Einstein-Hilbert action, c.f. Eq. \eqref{eq:13}, the entropy of a black hole is given by
\begin{equation}\label{eq:69}
	S=\frac{c^{3}A}{4G\hbar}\ ,
\end{equation}
where the constants are displayed on purpose, to highlight the fact that quantum mechanics plays an important role in calculating this entropy, hence the appearance of $\hbar$. Notice that Eq. \eqref{eq:69} depends only on the surface area of the black hole event horizon, $A$. This is taken to be a hint towards holography, since a quantity defined \textit{a priori} on a $D$ dimensional manifold depends on a $D-1$ dimensional quantity. 

\par Defining entropy for a black hole requires one to reformulate the second law of thermodynamics, in what is called the generalized second law of thermodynamics \cite{Bekenstein:1973ur}. Since the event horizon and beyond are literally invisible areas, once and object (presumably possessing a given amount of entropy) falls inside a black hole, its entropy would ``vanish" for an external observer - thus decreasing, which is clearly against the second law of thermodynamics. Hence the generalized second law, which states that the entropy for an ordinary system that falls into the black hole is compensated:
\begin{equation}\label{eq:70}
	\Delta S_{0}+\Delta S_{BH}\geq0\ ,
\end{equation}
with $\Delta S_{0}$ the change in entropy of the ordinary (exterior to the black hole) system.

\par Finally, the third law of thermodynamics (also called Nerst law) is still object of debate when it comes to the black hole scenario. In one of its forms, Nerst-Simon statement of the third law, it asserts ``the entropy of a system at absolute zero temperature either vanishes or becomes independent of its intensive thermodynamic parameters". It can be shown that for the Kerr-Newman black hole this is, at leat theoretically, not true. In the extremal case, where the sum of angular momentum density and electric charge are equal to the mass, one finds zero temperature without vanishing entropy. Moreover, the entropy depends on the angular momentum density, which from the first law, c.f. Eq. \eqref{eq:68}, can be identified with an intensive variable of the system. Theory aside, experimental tests have shown that the statement of the third law is unattainable by black holes, because the extremal condition is never met in real astrophysical scenarios.% [Thorne, K. S.: Talk at Texas Symposium on Relativistic Astrophysics, New York (1972)].

\subsubsection*{Thermodynamics of Reissner-Nordstr\"om black hole}
\par To end this section some explicit calculations regarding the thermodynamics of RN black holes are shown. This is not only instructive but will be important in later chapters, hence it also accounts for future reference. Notice that the RN black hole is the simplest case in which an extremal black hole can be defined, thus one can verify explicitly the statement regarding the third law, made in the last paragraph.

\par To avoid the need of introducing other coordinate systems one can make use of the first law of black hole mechanics, Eq. \eqref{eq:68}, to evaluate the temperature. To use such expression one needs the entropy, which, under adoption of natural units $c=G=\hbar=1$ is seen to be proportional to the area of the black hole. The RN black hole has spherical horizons, and as seen previously the outermost is $r_+$, c.f. Eq. \eqref{eq:63}. The area is simply
\begin{equation}\label{eq:71}
	A=4\pi r_+^2=4\pi\left(M+\sqrt{M^2-Q^2}\right)^2\ ,
\end{equation}
so the entropy of the RN black hole is
\begin{equation}\label{eq:72}
	S=\pi r_+^2=\pi\left(M+\sqrt{M^2-Q^2}\right)^2\ .
\end{equation}
Notice how $S=\pi Q^2$ on the extremal case, i.e. non-zero.

\par Writing the first law in a slightly different way
\begin{equation}\label{eq:73}
	TdS=dM-\Phi dQ\ ,
\end{equation}
where usage of Eqs. \eqref{eq:66} and \eqref{eq:69} has been made. Varying the entropy given by Eq. \eqref{eq:72}
\begin{equation}\label{eq:74}
	dS=\left(\frac{\partial S}{\partial M}\right)_{Q}dM+\left(\frac{\partial S}{\partial Q}\right)_{M}dQ\ ,
\end{equation}
where standard notation of thermodynamics is used. It is straight forward to check that
\begin{align}
\begin{aligned}\label{eq:75}
\frac{\partial S}{\partial M}&=2\pi\frac{\left(M+\sqrt{M^{2}-Q^{2}}\right)^{2}}{\sqrt{M^{2}-Q^{2}}}\\
\frac{\partial S}{\partial Q}&=-2\pi Q\frac{\left(M+\sqrt{M^{2}-Q^{2}}\right)}{\sqrt{M^{2}-Q^{2}}}
\end{aligned}
\end{align}
Comparing Eqs. \eqref{eq:74} with \eqref{eq:73} and using Eq. \eqref{eq:75} one finds that
\begin{equation}\label{eq:76}
	T=\frac{\sqrt{M^{2}-Q^{2}}}{2\pi\left(M+\sqrt{M^{2}-Q^{2}}\right)^{2}}\ .
\end{equation}
The surface gravity can be read off immediately by multiplying Eq. \eqref{eq:76} by $2\pi$. In doing this procedure one also finds the electric potential
\begin{equation}\label{eq:77}
	\Phi=\frac{Q}{M+\sqrt{M^2-Q^2}}=\frac{Q}{r_+}\ ,
\end{equation}
which was a result already known from solving Maxwell's equations.

\par An intriguing feature emerges from this calculation when the extremal case, i.e. $M=Q$, is considered, which is a non-zero entropy for vanishing temperature. In the context of holography such property gained a lot of attention in the recent years, and the theory dual to the RN black hole in the AdS background is interesting on its own, and shall be discussed in the next chapters. For now we just notice this as a matter of curiosity.

\par There are other ways of computing the temperature, namely introducing the imaginary time and demanding it be regular (this can be found at \cite{Nastase:2017cxp} ), and by direct application of Eq. \eqref{eq:66} once the coordinates are changed to the so called Eddington-Finkelstein coordinate system, which makes the radial and temporal coordinates regular at the horizon (for those interested in this route, it is done at \cite{Raine:2005bs}). Both of these methods arrive at the same expression, Eq. \eqref{eq:76}, but would require the introduction of more mathematical machinery.% and in fact, when a more complicated metric which shall introduce in the future comes into play those techniques are of no use due to specific properties of that space-time.


==> chapters/Intro.tex <==
\chapter{Introduction}
\par This work consists of mostly a review of various topics, aiming the understanding of how one can perform computations of transport coefficients using the AdS/CFT correspondence. The transport coefficients express how a system reacts when certain sources (test fields, in AdS/CFT context) interact with the system itself, a basic example is a charged system interacting with an electric field: one expects the charges to start moving along the electric field lines. In this simple example the charged particles represent the system, while the electric field is the source. The result of such interaction is an electric current and, how big or small the current is going to be depends on features of the system itself, the quantity that encodes these properties is called the electric conductivity, which is a transport coefficient.

\par More generally, to each source stimulating an interaction with a given system, one is able to define a transport coefficient. These are very important in Condensed Matter Physics, a particularly interesting example are superconductors at high temperature. Knowing how a given material behaves under specific circumstances allows one to study and understand how and why superconductivity happens. The same reasoning can be applied to superfluidity and plasma physicis, for example.

\par A problem that persists in condensed matter physics, in particular to systems mentioned above, is the description of strongly coupled systems. It is, in fact, a problem, because in this regime one is not able to apply the usual perturbation techniques - which is the analytic tool available to extract predictions from these systems from a theoretical standpoint. Thus, one has to rely mostly on numeric simulations, which have their own limitations.

\par The AdS/CFT correspondence changed this paradigm in the past decade. In fact, it has started a whole new research area, where theorists from many different areas of physics were able to contribute. This is because the AdS/CFT duality relates string theory to conformal field theory, and, in a specific limit this duality comes in handy to describe condensed matter system that cannot be described otherwise. Specifically, the duality relates weakly coupled super-gravity theories to strongly coupled conformal field theories in a specific regimes and, since the weakly coupled partner is being studied for a long time by string theorists, this area grew rapidly and many new phenomena, unpredicted otherwise, were called to attention.

\par To understand how computations using the AdS/CFT can be done, one has to understand the correspondence itself and the limitations that come with it, as well as the background theories that ``gravitate" around the correspondence, such as General Relativity and black hole thermodynamics, Conformal Field Theory, Gauge theories and, of course, Condensed Matter Theory in order to practically understand the results from computations. Besides the latter, the other subjects mentioned are discussed in this work, and external references to pioneering work in each of the areas are mentioned as well, since each of the subjects correspond to a research area on its own. The goal is to understand how all these theories fit into the AdS/CFT correspondence and hence, how one is able to use it, or at least identify it during computations.

\par The work is organized as follows: The first part is devoted to General Relativity, from Einstein-Hilbert action to black hole thermodynamics, going through some of the mathematics needed to obtain the solutions. The second part is called Review of AdS/CFT, where other topics such as conformal field theories and gauge theories are treated shortly, in fact, only the necessary parts of each subject that is needed to formulate the AdS/CFT correspondence and the GKPW relation, which is the great achievement of the correspondence and what enables one to obtain the results in strongly coupled field theories from knowledge of solutions from General Relativity. In the third part the Kubo relation is introduced and, through an example, it is shown how it can be used along with AdS/CFT to compute transport coefficients. Part four constitutes of a work published by the author with colleagues, and is a work in progress, so more results are expected. It is basically an application of what is discussed in the previous parts. At the end some perspectives are drawn, and expected results are outlined from knowledge obtained up to now.
